Radio haloes in nearby galaxies modelled with 1D cosmic-ray transport using SPINNAKER

We present radio continuum maps of 12 nearby ($D\leq 27~\rm Mpc$), edge-on ($i\geq 76^{\circ}$), late-type spiral galaxies mostly at $1.4$ and 5 GHz, observed with the Australia Telescope Compact Array, Very Large Array, Westerbork Synthesis Radio Telescope, Effelsberg 100-m and Parkes 64-m telescopes. All galaxies show clear evidence of radio haloes, including the first detection in the Magellanic-type galaxy NGC 55. In 11 galaxies, we find a thin and a thick disc that can be better fitted by exponential rather than Gaussian functions. We fit our SPINNAKER (SPectral INdex Numerical Analysis of K(c)osmic-ray Electron Radio-emission) 1D cosmic-ray transport models to the vertical model profiles of the non-thermal intensity and to the non-thermal radio spectral index in the halo. We simultaneously fit for the advection speed (or diffusion coefficient) and magnetic field scale height. In the thick disc, the magnetic field scale heights range from 2 to 8 kpc with an average across the sample of $3.0\pm 1.7~\rm kpc$; they show no correlation with either star-formation rate (SFR), SFR surface density ($\Sigma_{\rm SFR}$) or rotation speed ($V_{\rm rot}$). The advection speeds range from 100 to $700~\rm km\,s^{-1}$ and display correlations of $V\propto \rm SFR^{0.36\pm 0.06}$ and $V\propto \Sigma_{\rm SFR}^{0.39\pm 0.09}$; they agree remarkably well with the escape velocities ($0.5\leq V/V_{\rm esc}\leq 2$), which can be explained by cosmic-ray driven winds. Radio haloes show the presence of disc winds in galaxies with $\Sigma_{\rm SFR} > 10^{-3}~\rm M_{\odot}\,yr^{-1}\,kpc^{-2}$ that extend over several kpc and are driven by processes related to the distributed star formation in the disc.

==> tab8.tex <==
\begin{table}
\centering
\caption{Soft X-ray emission scale height $h_{\rm Xray}$ in the northern (N) and southern (S) halo.\label{tab:x-ray}}
\begin{tabular}{l cc c}
\hline
Galaxy & $h_{\rm Xray}$ (N) & $h_{\rm Xray}$ (S) & Reference\\
& (kpc) & (kpc) & \\\hline
NGC 55 & $(1.1^{+0.6}_{-0.4})$ & $(1.1^{+0.6}_{-0.4})$ & \citet{stobbart_06a}\\
NGC 253 & $2.1^{+1.2}_{-0.7}$ & $0.9^{+0.1}_{-0.1}$ & \citet{strickland_04a}\\
NGC 891 & $1.4^{+1.5}_{-0.4}$ & $2.0^{+0.6}_{-0.5}$& \citet{strickland_04a}\\
NGC 3079 & $3.7^{+1.0}_{-0.8}$ & $6.0^{+1.5}_{-1.1}$ & \citet{strickland_04a}\\
NGC 3628 & $1.6^{+0.2}_{-0.2}$ & $3.3^{+0.9}_{-0.7}$ & \citet{strickland_04a}\\
NGC 4631 & $2.2^{+0.2}_{-0.1}$ & $2.1^{+0.2}_{-0.2}$ & \citet{strickland_04a}\\
NGC 4666 & $4.6^{+2.3}_{-1.5}$ & $4.6^{+2.3}_{-1.5}$ & \citet{tuellmann_06a}\\
NGC 5775 & $3.9^{+2.0}_{-1.3}$ & $3.9^{+2.0}_{-1.3}$ & \citet{tuellmann_06a}\\
NGC 7090 & $(2.8^{+1.4}_{-0.9})$ & $(2.8^{+1.4}_{-0.9})$ & \citet{li_13a}\\
\hline
\end{tabular}
\flushleft{{\bf Notes.} Values from \citet{strickland_02a} are for $0.3$--$1.0$~keV and are corrected for our distances. Values from \citet{tuellmann_06a} are for $0.5$--$1.0$~keV and are estimated using their contour plots. Values from \citet{stobbart_06a} are for $0.3$--$1.0$~keV and \citet{li_13a} are for $0.5$--$1.5$~keV. Both are vertical extensions only and not scale heights.}
\end{table}

